Fake News Detection After LLM Laundering: Measurement and Explanation

With their advanced capabilities, Large Language Models (LLMs) can generate highly convincing and contextually relevant fake news, which can contribute to disseminating misinformation. Though there is much research on fake news detection for human-written text, the field of detecting LLM-generated fake news is still under-explored. This research measures the efficacy of detectors in identifying LLM-paraphrased fake news, in particular, determining whether adding a paraphrase step in the detection pipeline helps or impedes detection. This study contributes: (1) Detectors struggle to detect LLM-paraphrased fake news more than human-written text, (2) We find which models excel at which tasks (evading detection, paraphrasing to evade detection, and paraphrasing for semantic similarity). (3) Via LIME explanations, we discovered a possible reason for detection failures: sentiment shift. (4) We discover a worrisome trend for paraphrase quality measurement: samples that exhibit sentiment shift despite a high BERTSCORE. (5) We provide a pair of datasets augmenting existing datasets with paraphrase outputs and scores. The dataset is available on GitHub

==> documentBody/a-leftovers.tex <==
\section{LEFTOVERS}



%%%%%%%%%%%%%
Notes from chat with Andrew:

Normality - CLT be done with it (QQ plots can help) Table is bounded. The is skewed normal

Equivariance - we violate this

Welch’s T-test, welch’s ANOVA

Hedge’s g, could maybe get away with cohen’s d

Eta2 or partial eta2

Ramsey’s statistical sleuth, experimental design 


Finding of Hedge's test:
using this formula:
%g = (x1 – x2) / √((n1-1)*s12 + (n2-1)*s22) / (n1+n2-2)

% def hedges_g(group1, group2):
%     # Calculate means and standard deviations
%     mean1, mean2 = np.mean(group1), np.mean(group2)
%     std1, std2 = np.std(group1, ddof=1), np.std(group2, ddof=1)
%     n1, n2 = len(group1), len(group2)
    
%     # Calculate pooled standard deviation
%     pooled_std = sqrt(((n1 - 1) * std1**2 + (n2 - 1) * std2**2) / (n1 + n2 - 2))
    
%     # Calculate Cohen's d
%     hedges_g_value = (mean1 - mean2) / pooled_std
    
%     return hedges_g_value

    
Hedge's g: 0.3402894495157293 (Between GPT and llama)
Hedge's g: 1.7845745822763333 (Between Llama and Pegasus)
Hedge's g: 1.4679983117920334 (Between GPT and Pegasus)

Considerations:

\begin{itemize}
    \item Ensure the paraphrased versions retain the core message of the original fake news while varying in linguistic structure. Consider metrics like \textbf{BLEU}, \textbf{ROUGE}, and human evaluation to assess paraphrase quality.
    
    \item Address potential bias in paraphrasing models that might introduce artifacts, making the detection either easier or more challenging. 

    \item Choose a representative dataset of fake news for both training and testing, ensuring it covers various topics and styles. The dataset should be balanced to avoid skewing results.

    \item Consider which explainability methods are most appropriate for your models and how they can best illustrate differences in model behavior between human-written and paraphrased fake news.

    

    
\end{itemize}

%%%%%%%%%

% \\
% syntactic and/or lexical diversity and semantic similarity.\\
% The limited diversity and complexity in existing datasets restrict the ability of models.\\
% various applications on downstream NLP tasks, including \\
% * text summarization~\cite{cao2017joint},\\
% * semantic parsing~\cite{berant2014semantic},\\
% * diversifying text generation for user-facing systems like chatbots.\\
% * check the robustness of a model~\cite{iyyer2018adversarial}\\
% * question answering~\cite{fader2014open, yin2015answering}\\
% * data augmentation~\cite{yu2018qanet}
% * adversarial example generation~\cite{iyyer2018adversarial}



%\textbf{Challenge of paraphrasing}:\\
% Rephrasing the sentence while preserving the meaning but changing the syntactical or lexical form.

% \textbf{importance of comparative analysis of the paraphrasers}\\
% hinders the objective assessment of model performance\\
% making it challenging to identify strengths and weaknesses in existing approaches. \\
% impeding the development of improved models. \\
% also need to add from the Fake news perspective. \\

% What is a good paraphraser?
% 1) convey the same meaning
% 2) grammatically correct

% \begin{itemize}
%     \item Present a paraphrased dataset???
%     \item depending on results, we need to follow up on "why this research" with a contribution in that lane
% \end{itemize}

    %\FIXME{I like this RQ too; only feedback is to consider tacking on "and why"}
    %\item[\textbf{RQ4}] How does the quality of paraphrased text influence the effectiveness of fake news detection models?
    %\FIXME{Not sure I understand the qualitative part here. As I understand it, the experiment would proceed as such:
    %Classify original versions
    %Paraphrase original versions, noting paraphrase quality metrics
    %Classify paraphrased versions
    %Compare the distribution of paraphrase quality for (1) instances where original and paraphrased classifications differ with (2) all instances, maybe the complementary set.
    %}

%To find out which language model generated high quality paraphrases, we plotted the distribution of the Bertscore F1 score.
%A higher F1 score indicates more semantic similarity between the human-written and LLM-paraphrased texts.

Figure~\ref{covid_bertscore} demonstrates the distribution for the \covid{} dataset.
GPT demonstrates a broader distribution, peaking at a high F1 score of around 0.85 and spanning from 0.7 to 0.97. 
Llama also has a broader distribution, ranging from 0.7 to 0.95, with a peak around 0.84.
Pegasus exhibits a range spanning from 0.65 to 0.9 and peaks at a frequency higher than Llama around the 0.74 mark.


On the other hand, Figure~\ref{liar_bertscore} shows the \fbert{} calculated F1 score distribution for the LIAR dataset.
GPT's distribution shows a sharp peak around a high score of 0.90 and spans a relatively narrow range from approximately 0.85 to 0.95.
This indicates that GPT consistently produces paraphrases with high semantic similarity.
In contrast, while maintaining good performance, Llama's distribution has a broader spread from about 0.75 to 0.95, with a peak around 0.88, suggesting more variability in its output.
Pegasus has the broadest range of all, stretching from 0.75 to 1.00 with a peak at 0.80, indicating the least reliability; although it can achieve perfect scores, it also produces many lower scores.


Our findings demonstrate a significant performance difference in fake news detectors between human-written and LLM-paraphrased news content. 
The fake news detectors struggle to identify the LLM-paraphrased news articles than the human-written fake news articles.
For the LIAR dataset, LLM-paraphrased fake news, especially from Pegasus, poses the most challenges, with many models achieving low F1 scores, suggesting vulnerabilities to subtle paraphrasing.
Supervised models such as SVM with TF-IDF features show some resilience against GPT-paraphrased text, while deep-learning models such as LSTM and CNN struggle more with LLM-generated fake news.
In contrast, the \covid{} dataset shows more consistent results, with most detectors achieving high F1 scores on human-written content. 
However, Pegasus-generated paraphrases consistently emerge as the hardest to detect across both datasets.
These insights highlight the need for enhanced models capable of adapting to advanced paraphrasing techniques used for misinformation.


